Shifting Transformation Learning for Out-of-Distribution Detection

Detecting out-of-distribution (OOD) samples plays a key role in open-world and safety-critical applications such as autonomous systems and healthcare. Recently, self-supervised representation learning techniques (via contrastive learning and pretext learning) have shown effective in improving OOD detection. However, one major issue with such approaches is the choice of shifting transformations and pretext tasks which depends on the in-domain distribution. In this paper, we propose a simple framework that leverages a shifting transformation learning setting for learning multiple shifted representations of the training set for improved OOD detection. To address the problem of selecting optimal shifting transformation and pretext tasks, we propose a simple mechanism for automatically selecting the transformations and modulating their effect on representation learning without requiring any OOD training samples. In extensive experiments, we show that our simple framework outperforms state-of-the-art OOD detection models on several image datasets. We also characterize the criteria for a desirable OOD detector for real-world applications and demonstrate the efficacy of our proposed technique against state-of-the-art OOD detection techniques.

==> figures/head-count.tex <==

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/cifar10-head-count.PNG}}
\caption{Averaged OOD detection performance on number of self-supervised transformations in CIFAR-10 multi-class classification.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

==> figures/roc-figure.tex <==

\begin{figure}[t]
\vskip 0.1in
\begin{center}

    \begin{subfigure}[b]{0.49\columnwidth}
        \centerline{\includegraphics[width=1.1\columnwidth]{figures/our+SSL+CSI+SupSimCLRcifar10.pdf}}
        \caption{CIFAR-10 $D_{in}$} 
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
        \centerline{\includegraphics[width=1.1\columnwidth]{figures/our+SSL+CSI+SupSimCLRcifar100.pdf}}
        \caption{CIFAR-100 $D_{in}$}
    \end{subfigure}
\caption{Comparison between different OOD detection methods when  $D_{test}^{out}$ is mix of six disjoint outlier datasets. 
% Detectors without generalized OOD feature learning (i.e., ODIN and Mahanalobis) show significant performance drop when facing mix of outlier distributions.
% Comparison of OOD detection ROC curves from all zero-shot techniques trained on CIFAR10 and CIFAR100 datasets and mixture of 6 disjoint sets
}
\label{fig:roc}
\end{center}
\vskip -0.2in
\end{figure}



==> figures/trainin-weights.tex <==

\begin{figure}[t]
\vskip 0.1in
\begin{center}
    \begin{subfigure}[b]{0.32\columnwidth}
        \centerline{\includegraphics[width=0.97\columnwidth]{figures/w-cifar10-7.png}}
        \caption{CIFAR-10 Training Set}%  as in-distribution
    \end{subfigure}
    \begin{subfigure}[b]{0.32\columnwidth}
        \centerline{\includegraphics[width=0.97\columnwidth]{figures/w-cifar100-7.png}}
        \caption{CIFAR-100 Training Set} %  OOD detection results on  ... as in-distribution
    \end{subfigure}
    \begin{subfigure}[b]{0.32\columnwidth}
        \centerline{\includegraphics[width=0.97\columnwidth]{figures/w-imagenet-7.PNG}}
        \caption{ImageNet-30 Training Set} %  as in-distribution
    \end{subfigure}
\caption{\TODO{update colors} Ablation study to measure effects of individual and paired transformations on OOD detection performance. Experiments are done on CIFAR-10 \textbf{(top)} and CIFAR-100 \textbf{(bottom)} multi-class classification setup. % The OOD test sets are CIFAR-100 (top) and CIFAR-10 (bottom) experiments. 
Results indicate that the choice of effective transformations depends on the in-domain training set. % \revised{and network}.
}
\label{fig:lambda-weights}
\end{center}
\vskip -0.2in
\end{figure}



==> sections/method-old.tex <==




\vspace{-0.5em}
\section{Method}
\label{sec:method}

\vspace{-0.5em}
Learning invariances with identity-preserving transformations is a technique to incorporate prior knowledge to improve representation learning and hence OOD detection. 
However, training an invariant network is challenging, and common data augmentation techniques do not guarantee for that \cite{lyle2020benefits} and may even degrade training performance \cite{chen2020simple}.
To address this issue, Tack et al. \cite{tack2020csi} suggested to use some augmentations as negative samples in contrastive training, Xiao et al. \cite{xiao2021what} proposed using multiple embedding sub-spaces for each augmentation, and Lee et al. \cite{lee2020self} use label augmentation to train for image invariances. 
In contrast to these work, we suggest using multi-task learning for explicit and efficient training of a wide range of invariances to in-domain representations. 
Intuitively, we simultaneously train the base encoder on \textit{multiple shifted distributions} of the training data using auxiliary self-supervised objectives for unlabeled data and fully-supervised objectives for labeled data.
In Sec.~\ref{sec:losses}, we present our multi-task transformation learning objective, in Sec.~\ref{sec:method-opt}, we present a simple method for selecting optimal transformation and controlling their impact on representation learning, and in Sec.~\ref{sec:scores}, we discuss our detection score.



% ---------------------------------------------
\input{figures/trans-set-and-weights}
% --------------------------------------------


\subsection{Multi-task Transformation Learning} \label{sec:losses}
\vspace{-0.25em}
Our transformation learning technique trains a multi-tasked network using self-supervised and fully-supervised training objectives. We consider a set of geometric (translation, rotation) and non-geometric (blurring, sharpening, color jittering, Gaussian noise, cutout) transformations and we train the network with dedicated loss functions for each transformation.  
For the self-supervised transformation learning, given an unlabeled training set of  $\mathcal{S} = \{(x_i)\}_{i=1}^{M}$, we denote the set of domain invariant transformations $T_{n}$ by $\mathcal{T} = \{T_{n}\}_{n=1}^N$.
We generate a self-labeled training set $\mathcal{S}_{T_{n}} = \{(T_{n}(x_{i}), \hat{y}_{i})\}_{i=1}^M$ for each self-supervised transformation $T_{n}$ where $\hat{y}_{i}$ are the transformation labels. 
For example, we consider the image rotation task with four levels of \{0$^{\circ}$, 90$^{\circ}$, 180$^{\circ}$, 270$^{\circ}$\} self-labeled rotations and $\hat{y}_{i} \in \{0, 1, 2, 3\}$ in this case.
The self-supervised loss $\mathcal{L}_{\text{ssl}}$ is the weighted average of loss across all transformations in $\mathcal{T}$:
%
%
\begin{equation} \label{eq:eq_ssl}
\mathcal{L}_{\text{ssl}}(\blambda, \btheta) = \frac{1}{N} \sum_{n=1}^{N} \lambda_{n} \sum_{(T_{n}(x_{i}), \hat{y}_{i}) \in S_{T_{n}}} \ell (f^{(n)}_\btheta(T_n({x_{i})}),\hat{y_i}),     
\end{equation}
%
%
where $f^{(n)}_\btheta$ is a classification network with parameters $\btheta$ for the $n^{th}$ task and $\blambda = \{\lambda_n\}_{n=1}^N$ are transformation weights. 
%
% -------------------------------------------
\input{algs/main-alg}
% -------------------------------------------
%
When labels are available, given the labeled training set of  $\mathcal{S} = \{(x_i, y_i)\}_{i=1}^{M}$, we generate transformed copies of the original training sets $\mathcal{S}_{T_{n}} = \{(T_{n}(x_{i}), y_i)\}_{i=1}^M$ where the samples retain original class labels. 
The supervised loss $\mathcal{L}_{\text{sup}}$ is defined by: %the total of classification loss on the weighted average of transformed copies of the training set:
%
%\sum_{(x_{i}, y_i) \in S} \ell (f'^{(0)}_\btheta(x_{i}),y_i) 
\begin{equation} \label{eq:eq_sup}
\mathcal{L}_{\text{sup}}(\blambda', \btheta) = \lambda'_{0}   \mathcal{L}_{\text{main}}(\btheta) + \frac{1}{N} \sum_{n=1}^{N} \lambda_{n}' \sum_{(T_{n}(x_{i}), y_i) \in S_{T_{n}}} \ell (f'^{(n)}_\btheta(T_n({x_{i})}),y_i),    
\end{equation} 
%
%
% The supervised loss $\mathcal{L}_{\text{sup}}$ is the total of classification loss on the clean set and weighted average of loss across all transformed copied of training set: 
% \begin{equation} \label{eq:only_eq_2}
% \mathcal{L}_{\text{sup}} = \lambda_{0}\sum_{(x_i,y_i) \in S} \ell (f^{(n)}_\btheta(x_i),y_i)  + \frac{1}{N} \sum_{n=1}^{N} \lambda_{n} \sum_{(T_{n}(x_{i}), y_i) \in S_{T_{n}}} \ell (f^{(n)}_\btheta(T_n({x_{i})}),y_i)     
% \end{equation} 
%
%
% where the first summation measures the main classification loss and 
where the $\mathcal{L}_{\text{main}}(\btheta)$ is any main supervised learning task and the second summation measures the classification loss for transformed copies of the data. 
$\blambda' = \{\lambda'_n\}_{n=0}^N$ are transformation coefficients in $\mathcal{L}_{\text{sup}}$.
In the rest of the paper, for the ease of notation, we use $\Lambda$ to refer to all the transformation coefficients set $\Lambda =  \{\blambda, \blambda'\}$. % , and we drop $\blambda', \btheta$ when it is clear from the context.
When labels are available, we define the auxiliary transformation loss as $\mathcal{L}_{\text{aux.}} := \mathcal{L}_{\text{ssl}} + \mathcal{L}_{\text{sup}}$, otherwise we define $\mathcal{L}_{\text{aux.}} := \mathcal{L}_{\text{ssl}}$ using only the self-supervised loss.
% \draft{where $\blambda = \{\lambda_n\}_{n=0}^{2N}$ are transformation coefficients for both $\mathcal{L}_{\text{sup}}$ and $\mathcal{L}_{\text{ssl}}$.} 
\iffalse
In supervised learning, we can combine (\ref{eq:eq_ssl}) and (\ref{eq:eq_sup}) to benefit from hybrid training of both self-supervised and fully-supervised learning of transformations: 
%
%
\begin{equation} \label{eq:eq_hybrid}
\mathcal{L}_{\text{hybrid}} = \mathcal{L}_{\text{sup}} + \mathcal{L}_{\text{ssl}}
\end{equation}
%
%
% \AV{Should we change $\mathcal{L}_{\text{hybrid}} \rightarrow \mathcal{L}_{\text{trans.}}$ or the other way around?}
\fi
%The auxiliary transformation learning loss $\mathcal{L}_{\text{aux.}}$ can be combined with any main learning tasks $\mathcal{L}_{\text{main}}$ (e.g., image classification loss) for improved OOD detection using $\mathcal{L}_{\text{total}}(\blambda', \btheta) = \mathcal{L}_{\text{main}}(\blambda', \btheta) + \lambda_{0}\mathcal{L}_{\text{aux.}}(\blambda', \btheta)$,
% \AV{robustness or detection?}: %  improve representation learning and hence OOD detection: 
%$\mathcal{L}_{\text{sup}}$ in (\ref{eq:eq_sup})
%
%\begin{equation} \label{eq:eq_total}
%\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{main}} + %\lambda_{0}\mathcal{L}_{\text{aux.}} 
%\end{equation}
%
%
% \begin{equation}
% \mathcal{L}_{\text{main}} = \sum_{(x_i,y_i) \in S} \ell (f^{(n)}_\btheta(x_i),y_i)  \label{eq:main_task}
% \end{equation}
%
%
%where $\lambda_{0}$ is the trade-off coefficient between the main task (on clean training set) and auxiliary transformation learning tasks.

Instead of training a separate network $f^{(n)}_\btheta$ or $f'^{(n)}_\btheta$ for each task, all the auxiliary tasks and the main classification task share the a feature extraction network and each only introduces an additional 2-layer fully-connected head for each task. Training is done in a multi-task fashion in which the network is simultaneously trained for the main classification (if applicable) and all weighted auxiliary tasks using the cross-entropy loss. 
% Transformations are applied to individual small mini-batches and unlike contrastive learning are 



% % ------------------------------------------
% \input{figures/trainin-weights}
% % ------------------------------------------



\vspace{-0.5em}
\subsection{Learning to Select Transformations} 
\label{sec:method-opt}
\vspace{-0.25em}
Previous work on self-supervised learning used ad-hoc heuristics for choosing data transformations for the training set \cite{Hendrycks2019sv,golan2018deep,tack2020csi}.
However, the choice of effective transformation(s) depends on the source distribution and heuristic approaches cannot scale up to diverse training distributions when there are many potential transformations to consider. 
To illustrates this, we train a ResNet-18 \cite{he2016deep} with single and paired self-supervised transformations that are selected from a pool of seven transformations.  
The OOD detection results are reported in Figure \ref{fig:all-trans}-top with CIFAR-10, CIFAR-100 \cite{krizhevsky2009learning}, and ImageNet-30 \cite{Hendrycks2019sv} datasets as in-distribution and CIFAR-100, CIFAR-10, and Pets \cite{parkhi2012cats} as OOD test sets, respectively.
The heatmap visualization presents a clear view of how different transformations (and the combinations of two) have a different impact on the OOD detection performance depending on the source distribution.
For example, although rotation is the most effective transformation on CIFAR-10 and ImageNet-30, it is among the least effective ones for CIFAR-100. On the other hand, sharpening and color jittering are from the most effective transformations for CIFAR-100, but they perform worse on CIFAR-10. 
% \paragraph{Transformations Selection Framework:} 
From these observations, we propose a simple framework that relies on Bayesian optimization to first select effective transformation set $\mathcal{T}$, and then it uses meta-learning to learn optimum $\blambda$ weights for OOD robustness. %Note that since we assume that we do not have access to the target OOD distribution(s), we only rely on $\mathcal{L}_{\text{ssl}}$ or $\mathcal{L}_{\text{hybrid}}$ for labeled training sets as the optimization objective. 
% Note that the order $\mathcal{T}$ selection and  $\blambda$ matters as the Bayesian optimization was more successful in capturing the long term effect of transformation learning. 
% \draft{Algorithm 1 presents the framework for unlabeled training sets.} % \ref{alg:only_alg}




\noindent \textbf{Optimizing Transformations Set $\mathcal{T}$:} We use Bayesian optimization to identify effective transformations for each in-domain training set as shown in Alg.~\ref{alg:bayesian}. Here, we assume that transformation weights $\blambda$ are one and we only search for effective transformations set from a pool of available transformations.
% Our results show that Bayesian optimization can capture the direct effect of transformations set $\mathcal{T}$ on representation learning very well. 
We use a low-cost off-the-shelf Bayesian optimization \cite{akiba2019optuna} library to find the optimum self-supervised task set due to the small $\mathcal{T}$ search space (i.e., $2^n$ for the $\mathcal{T}$ set of $n$). 
%The optimization objective is to minimize the transformation learning loss ($\mathcal{L}_{\text{ssl}}$ for unlabeled test set and $\mathcal{L}_{\text{hybrid}}$ for unlabeled test set) on the available $D_{val}^{in}$.
The Bayesian optimization objective seeks to minimize the transformation learning loss $\mathcal{L}_{\text{aux.}}$ on the available $D_{val}^{in}$. 
% \AV{$D_{val}^{in}$ or $D_{val}^{in}$}


\noindent \textbf{Optimizing Transformations Weights $\blambda$:}  Next, we optimize $\blambda$ coefficients for the selected transformation from the previous step to further improve representation learning. 
This is important because the $\blambda$ coefficients modulate the impact of different transformations in the training objective in Eq.~\ref{eq:eq_ssl} and Eq.~\ref{eq:eq_sup}. 
Here, we assume that $\blambda$ is a ``meta-parameter'' and we use a differentiable hyperparameter optimization algorithm~\cite{maclaurin2015gradient} for optimizing it as shown in Alg.~\ref{alg:only_alg}. 
Our optimization algorithm consists of an inner training updates that trains network parameters $\btheta$ using $\mathcal{L}_{\text{sup}}$ on $D_{train}^{in}$ for $K$ steps. 
Given the current state of parameters $\btheta$, we update $\blambda$ in the outer loop such that $\mathcal{L}_{\text{main}}(\btheta)$ is minimized on $D_{val}^{in}$. Note that the gradient of $\mathcal{L}_{\text{main}}(\btheta)$ w.r.t. $\Lambda$ is defined only through the gradient updates in the inner loop. Thus, the $\Lambda$ update in the outer loop requires backpropagating through the gradients updates in the inner loop which can be done using differentiable optimizers~\cite{grefenstette2019generalized}.

We use $K=1$ step for the inner-loop optimization with SGD when updating $\btheta$ and we use Adam \cite{kingma2014adam} to update $\blambda$. Figure \ref{fig:all-trans}-bottom presents $\blambda$ values during optimization from an ablation study on three training sets and reveals the dependency and importance of optimum $\blambda$ weights. 





\iffalse
We add $\blambda$ training coefficients to the model $f$ parameters and choose the $\mathcal{L}_{\text{ssl.}}$ from Eq. \ref{eq:eq_ssl} (or $\mathcal{L}_{\text{hybrid}}$ Eq. \ref{eq:eq_hybrid} if labels available) as the minimization objective. 
After equal $\lambda_n = 1$ initialization for all transformation tasks, we calculate the validation loss gradients $\nabla_{\lambda_n} \ell (f_{\lambda_n}(T_n({x_{i})}),\hat{y_i}) $ 
% $\nabla_{\lambda_n} \mathcal{L}_{trans.} (f_{\lambda_n})$ 
with respect to each task (i.e. each $\blambda$ ``meta-parameters''). 
Then, given learning rate hyperparameters $(\alpha,\beta)$, we compute adapted meta-parameters $\lambda_n' = \lambda_n - \alpha\nabla_{\lambda_n} \ell (f_{\lambda_n}(T_n({x_{i})}),\hat{y_i}) $ for each task in an inner loop. 
Finally, we update parameters with the  concatenation of
meta-outputs on all training task $\lambda_n \leftarrow \lambda_n - \beta\nabla_{\lambda_n} \sum f_{\lambda_n}(T_n({x_{i})}),\hat{y_i}$ with gradient descent. 
\fi



\vspace{-0.5em}
\subsection{Detection Scores} \label{sec:scores}
\vspace{-0.5em}
We consider two techniques for computing network output: (i) We can aggregate the softmax prediction from the main task and all auxiliary transformation heads to compute an \textit{ensemble score}. (ii) Alternatively, if the computational budget is limited for OOD detection, a fast detection score can be computed using the main classification head while discarding auxiliary transformation heads after training (see Table \ref{tab:tiny-ens} for comparison). 
Given softmax scores obtained from either (i) or (ii), we use KL divergence between the softmax prediction and uniform distribution \cite{Hendrycks2019sv} as the OOD detection score.
% examine three detection scores including maximum softmax prediction~\cite{hendrycks2016baseline}, entropy of the softmax prediction~\cite{mohseni2020ood}, and KL divergence between the softmax prediction and uniform distribution \cite{Hendrycks2019sv}. 
Unless mentioned otherwise, our main evaluation results are based on the ensembled score from available auxiliary heads. %  for all unlabeled and one-class detection.

==> tables/normal-acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% columnwidth


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}

% \begin{wraptable}{r}{5.5cm}
% \caption{A wrapped table going nicely inside the text.}\label{wrap-tab:1}
% \begin{tabular}{ccc}\\\toprule  
% Header-1 & Header-1 & Header-1 \\\midrule
% 2 &3 & 5\\  \midrule
% 2 &3 & 5\\  \midrule
% 2 &3 & 5\\  \bottomrule
% \end{tabular}
% \end{wraptable} 

% \begin{table}[]
\begin{wraptable}{r}{11cm}
\centering
\caption{Comparison of classification accuracy between fully supervised Baseline and state-of-the-art self-supervised techniques trained on WideResNet-40-2 (2.2M parameters) and ResNet-18 (11.7M parameters) networks.}
% \caption{Comparison of classification accuracy between fully supervised (Baseline), geometric self-supervised learning (Geometric), supervised contrastive learning (SupSimCLR), and shifting contrastive learning (CSI) trained on WideResNet-40-2 (2.2M parameters) and ResNet-18 (11.7M parameters) networks.}
\label{tab:normal-acc}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccc@{}}
\cmidrule(l){2-4}
\multirow{2}{*}{} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}WideResNet-40-2\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet-18\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet-50\end{tabular}} \\ \cmidrule(l){2-4} 
 & CIFAR10/100 & CIFAR10/100 \\ \midrule
Baseline \cite{hendrycks2016baseline} & 92.10\%/69.59\% & 94.53\%/75.78\% & xx.xx\%/xx.xx\% \\
Geomtric \cite{hendrycks2019using}  & 93.57\%/71.61\% & 94.86\%/74.07\% & xx.xx\%/xx.xx\%\\
SupSimCLR \cite{yu2019unsupervised} & 94.80\%/73.31\% & 94.47\%/73.53\% & xx.xx\%/xx.xx\%\\
CSI \cite{tack2020csi} & 94.33\%/69.79\% & 94.75\%/76.12\% & xx.xx\%/xx.xx\%\\
Our & \textbf{95.80\%}/\textbf{77.12\%} & \textbf{96.07\%}/\textbf{77.94\%} & xx.xx\%/xx.xx\%\\ \bottomrule
\end{tabular}%
% }
% \end{table}
\end{wraptable} 
% ---------------------------------------------------------
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% % \caption{Comparison of models' main classification accuracy (\%) trained on ResNet-18 and WideResNet-40-2 networks to learn geometric and non-geometric invariances: fully supervised (Baseline), geometric self-supervised learning \cite{hendrycks2019using} (Geometric), supervised contrastive learning \cite{khosla2020supervised} (SupSimCLR), and shifting contrastive learning \cite{tack2020csi} (CSI). \TODO{change the order based on network size}}
% \caption{Comparison of classification accuracy between fully supervised (Baseline), geometric self-supervised learning (Geometric), supervised contrastive learning (SupSimCLR), and shifting contrastive learning (CSI) trained on ResNet-18 and WideResNet-40-2 networks.}
% \label{tab:normal-acc}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{cc|c|cc}
%  & \multicolumn{2}{c|}{ResNet-18 (11.7M para.)} & \multicolumn{2}{c}{WideResNet-40-2 (2.2M para.)} \\ \cline{2-5} 
% \multicolumn{1}{c|}{} & CIFAR10 & CIFAR100 & \multicolumn{1}{c|}{CIFAR10} & CIFAR100 \\ \hline
% \multicolumn{1}{c|}{Baseline} & 94.53\% & 75.78\% & \multicolumn{1}{c|}{92.1\%} & 69.59\% \\
% \multicolumn{1}{c|}{Geometric} & 94.86\% & 74.07\% & \multicolumn{1}{c|}{93.57\%} & 71.61\% \\
% \multicolumn{1}{c|}{SupSimCLR} & 94.47\% & 73.53\% & \multicolumn{1}{c|}{94.8\%} & 73.3\% \\
% \multicolumn{1}{c|}{CSI} & 94.75\% & 76.12\% & \multicolumn{1}{c|}{94.3\%} & 69.7\% \\
% \multicolumn{1}{c|}{Our} & \textbf{96.07\%} & \textbf{77.94}\% & \multicolumn{1}{c|}{\textbf{95.80\%}} & \textbf{77.1}\%
% \end{tabular}
% }
% % \\ \colorbox{yellow}{or...}\\
% % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{c|c|c|c|c|c}
% %  & Baseline & \multicolumn{1}{l|}{Geometric} & SupSimCLR & CSI & Our \\ \cline{2-6} 
% % CIFAR10 & 94.53\% & 94.86\% & 94.47\% & 94.75\% & \textbf{96.07\%} \\
% % CIFAR100 & 75.78\% & 74.07\% & 73.53\% & 76.12\% & \textbf{77.94\%}
% % \end{tabular}%
% % }
% % \\ \colorbox{yellow}{or a line chart...}\\
% \end{table}

% % -------------------------------------------------
% \begin{table}[]
% \centering
% \caption{Comparison of model normal accuracy (\%) trained on a ResNet-18 network with different approaches to learn geometric and non-geometric invarances: fully supervised (Baseline), geometric self-supervised tasks \cite{hendrycks2019using} (Geometric), supervised contrastive learning \cite{khosla2020supervised} (SupSimCLR), and shifting contrastive learning \cite{tack2020csi} (CSI). }
% \label{tab:normal-acc}
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|c|c}
%  & CIFAR10 & \multicolumn{1}{c|}{CIFAR100} \\ \hline
% Baseline & 94.53\% & \multicolumn{1}{c|}{75.78\%} \\
% Geomtric & 94.86\% & \multicolumn{1}{c|}{74.07\%} \\
% SupSimCLR & 94.47\% & \multicolumn{1}{c|}{73.53\%} \\
% CSI & 94.75\% & \multicolumn{1}{c|}{76.12\%} \\
% Our & \textbf{96.07}\% & \multicolumn{1}{c|}{\textbf{77.94}\%}
% \end{tabular}%
% % }
% \end{table}


% \begin{table}[]
% \centering
% \caption{Comparison of model normal accuracy (\%) trained on a ResNet-18 network with different approaches to learn geometric and non-geometric invarances: fully supervised (Baseline), geometric self-supervised tasks \cite{hendrycks2019using} (Geometric), supervised contrastive learning \cite{khosla2020supervised} (SupSimCLR), and shifting contrastive learning \cite{tack2020csi} (CSI). }
% \label{tab:normal-acc}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|c|c|c|c|c}
%  & Baseline & \multicolumn{1}{l|}{Geometric} & SupSimCLR & CSI & Our \\ \cline{2-6} 
% CIFAR10 & 94.53\% & 94.86\% & 94.47\% & 94.75\% & 96.07\% \\
% CIFAR100 & 75.78\% & 74.07\% & 73.53\% & 76.12\% & 77.94\%
% \end{tabular}%
% }
% \end{table}

==> tables/perturbation_types.tex <==

\begin{figure}[H]
\vskip 0.00in
\begin{center}
\centerline{\includegraphics[width=0.99\columnwidth]{figures/pert_3.png}}
%     \centerline{\includegraphics[width=0.99\columnwidth]{figures/pert_1.png}}
% (a) Distance-based techniques
% \centerline{\includegraphics[width=0.99\columnwidth]{figures/pert_2.png}}
% (b) Classification-based techniques
% \textbf{(Left)} distance-based and \textbf{(Right)} Classification-based
\caption{OOD detection robustness results for state-of-the-art techniques. Both $D_{test}^{out}$ (TinyImageNet) and $D_{test}^{in}$ (CIFAR-10) are perturbed with 5 levels intensities. $\times$ sign shows the mean AUROC.} % {}\textsuperscript{\textdagger}{OE} requires additional $D_{train}^{out}$ set for training.
\label{fig:pert_types}
\end{center}
\vspace{-1.75em}
% \vskip -0.2in
\end{figure}

==> tables/summary-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Review of OOD detection criteria, averaged detection performance, and robustness under different mixed and shifted OOD test distributions (AUROC \%). We compare our technique with ODIN \cite{lee2017training}, Mahanalobis \cite{lee2018simple}, Outlier Exposure \cite{hendrycks2018deep} Geometric \cite{hendrycks2019using}, CSI \cite{tack2020csi}, and Gram \cite{sastry2019detecting}. The horizontal line separates results for zero-shot techniques from those that require OOD samples. Best results from zero-shot techniques are bolded.}
\label{tab:table-of-criteria}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccm{1mm}cc}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Detection \\ Technique\end{tabular}} & \multicolumn{3}{c}{OOD Detection Criteria} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Averaged \\ Detection \\ Performance\end{tabular}} & \multicolumn{3}{c}{Generalizability Tests} &\multirow{2}{*}{}& \multicolumn{2}{c}{Robustness Tests} \\ \cline{2-4} \cline{6-8} \cline{10-11} 
 & \begin{tabular}[c]{@{}c@{}}Hyp.-Para. \\ Dependency\end{tabular} & Generalizable & Zero-shot &  & \begin{tabular}[c]{@{}c@{}}Mixed-OOD\end{tabular} & Far-OOD & Near-OOD &  & Rotation Pert. & Noise Pert. \\ \hline
\multicolumn{1}{c|}{ODIN} & High & \textbf{--} & \textbf{--} & 91.15 & 88.10 & 96.70 & 85.80 && 77.9 & 84.76 \\
\multicolumn{1}{c|}{Mahanalobis} & High & \textbf{--} & \textbf{--} & 95.18 & 92.24 & 99.10 & 88.51 && 83.52 & 87.91 \\
\multicolumn{1}{c|}{Outlier Exposure} & Low & \ding{51} & \textbf{--} & 96.24 & 96.88 & 98.76 & 93.41 && 90.28 & 92.89 \\ \cline{1-11} 
\multicolumn{1}{c|}{Geometric} & Low & \ding{51} & \textbf{\ding{51}} & 94.05 & 94.29 & 97.96 & 91.91 && 89.07 & 53.20 \\
\multicolumn{1}{c|}{CSI} & Low & \ding{51} & \textbf{\ding{51}} & 94.07 & 93.81 & 96.11 & 90.60 && 83.29 & 43.69 \\
\multicolumn{1}{c|}{Gram Matrices} & No & \textbf{--} & \textbf{\ding{51}} & 94.17 & 95.08 & 99.50 & 79.01 && \textbf{91.71} & \textbf{86.58} \\
\multicolumn{1}{c|}{Ours} & No & \ding{51} & \textbf{\ding{51}} & \textbf{95.39} & \textbf{95.66} & \textbf{99.92} & \textbf{93.05} && 89.59 & 80.29
\end{tabular}%
}
\end{table*}
%  -------------------------------------------------------


==> tables/tiny_one_class.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Comparison of OOD detection results (AUROC \%) with different one-class classification and unlabeled multiclass datasets on CIFAR-10, CIFAR-100, and ImageNet-30.}
\label{tab:one-class}
\vspace{2mm}\par
(a) Unlabeled CIFAR-10, CIFAR-100, and ImageNet-30 %  \cite{Hendrycks2019sv} \cite{chen2020simple} \cite{sehwag2021ssd}  \cite{tack2020csi}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{cccccc}
\hline
$D^{in}$ & Geometric & SimCLR  & SSD  & CSI-ens & Ours ($\mathcal{L}_{\text{trans-ssl}}$) \\ \hline
\multicolumn{1}{c|}{CIFAR-10} & 86.04 & 77.84 & 84.54 & \textbf{91.99} & 89.9 \\
\multicolumn{1}{c|}{CIFAR-100} & 75.28 & 48.81 & 66.41 & 71.91 & \textbf{83.95} \\
\multicolumn{1}{c|}{ImageNet-30} & 85.30 & 67.91 & -- & 90.14 & \textbf{96.77} \\
\hline
\end{tabular}
}
\vspace{2mm}\par
(b) Unlabeled One-class Detection on CIFAR-10  % \cite{ruff2018deep} \cite{goyal2020drocc} \cite{bergman2020classification} \cite{Hendrycks2019sv}  \cite{sehwag2021ssd} \cite{chen2020simple}
\resizebox{0.5\textwidth}{!}{


\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One-class\\ Training sets \end{tabular}} & \multicolumn{5}{c}{One-Class Detection Performance (averaged AUROC)} \\ \cline{2-6} 
& Geometric & SimCLR  & CSI  & SSD   & Our method     \\ \hline
% \multicolumn{1}{c|}{SVHN}    & xx.xx      & xx.xx         & xx.xx & xx.xx            & \textbf{xx.xx}  \\
\multicolumn{1}{c|}{One Class CIFAR10}    & xx.xx     & xx.xx         & xx.xx & xx.xx            & \textbf{xx.xx}  \\ 
\multicolumn{1}{c|}{One Class ImageNet-30}    & xx.xx      & xx.xx         & xx.xx & xx.xx            & \textbf{xx.xx}  \\
\hline
\multicolumn{1}{c|}{Unlabeled CIFAR10}    & xx.xx     & xx.xx         & xx.xx & xx.xx            & \textbf{xx.xx}  \\ 
\multicolumn{1}{c|}{Unlabeled ImageNet-30}    & xx.xx      & xx.xx         & xx.xx & xx.xx            & \textbf{xx.xx}  
\end{tabular}

}
\end{table}






==> tables/x-table.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

